Learning a Behavior Model of Hybrid Systems Through Combining Model-Based Testing and Machine Learning (Full Version)

Models play an essential role in the design process of cyber-physical systems. They form the basis for simulation and analysis and help in identifying design problems as early as possible. However, the construction of models that comprise physical and digital behavior is challenging. Therefore, there is considerable interest in learning such hybrid behavior by means of machine learning which requires sufficient and representative training data covering the behavior of the physical system adequately. In this work, we exploit a combination of automata learning and model-based testing to generate sufficient training data fully automatically. Experimental results on a platooning scenario show that recurrent neural networks learned with this data achieved significantly better results compared to models learned from randomly generated data. In particular, the classification error for crash detection is reduced by a factor of five and a similar F1-score is obtained with up to three orders of magnitude fewer training samples.

==> Premeables/grants.tex <==
This work was supported by the Graz University of Technology's LEAD project
``Dependable Internet of Things in Adverse Environments''. 
It was also partially supported by the European Union (IMMORTAL, grant 644905), 
by the ECSEL Joint Undertaking (ENABLE-S3, grant 692455).

==> Results/CDFs/lbt.tex <==
\begin{tikzpicture}
    \node (200) {\input{Results/CDFs/lbt_200.tex}};
    \node[right=-1/4 of 200] (2k) {\input{Results/CDFs/lbt_2k.tex}};
    \node[right=-1/4 of 2k] (20k) {\input{Results/CDFs/lbt_20k.tex}};
    \node[right=-1/4 of 20k] (200k) {\input{Results/CDFs/lbt_200k.tex}};
\end{tikzpicture}

==> Results/CDFs/out.tex <==
\begin{tikzpicture}
    \node (200) {\input{Results/CDFs/out_200.tex}};
    \node[right=-1/4 of 200] (2k) {\input{Results/CDFs/out_2k.tex}};
    \node[right=-1/4 of 2k] (20k) {\input{Results/CDFs/out_20k.tex}};
    \node[right=-1/4 of 20k] (200k) {\input{Results/CDFs/out_200k.tex}};
\end{tikzpicture}

==> Results/CDFs/rand.tex <==
% \documentclass[tikz,border=5pt,multi=tikz,crop]{standalone}
% \newcommand{\ieee}[1]{}
% \newcommand{\lncs}[1]{}
% \newcommand{\acm}[1]{}
% \newcommand{\blind}[1]{}

% \usepackage{datatool}
% \usepackage{pgfplots}
% \usepackage{amsmath}
% \input{Premeables/packages.tex}
% \input{Premeables/defs.tex}
% \pgfplotsset{compat=1.12}

% \begin{document}
\begin{tikzpicture}
    \node (200) {\input{Results/CDFs/rand_200.tex}};
    \node[right=-1/4 of 200] (2k) {\input{Results/CDFs/rand_2k.tex}};
    \node[right=-1/4 of 2k] (20k) {\input{Results/CDFs/rand_20k.tex}};
    \node[right=-1/4 of 20k] (200k) {\input{Results/CDFs/rand_200k.tex}};
\end{tikzpicture}
% \end{document}

==> Results/CDFs/tc.tex <==
\begin{tikzpicture}
    \node (200) {\input{Results/CDFs/tc_200.tex}};
    \node[right=-1/4 of 200] (2k) {\input{Results/CDFs/tc_2k.tex}};
    \node[right=-1/4 of 2k] (20k) {\input{Results/CDFs/tc_20k.tex}};
    \node[right=-1/4 of 20k] (200k) {\input{Results/CDFs/tc_200k.tex}};
\end{tikzpicture}

==> Sections/introduction_old.tex <==
\section{Introduction}
\remove
{
The emergence of \ac{IoT} has made \acp{CPS} to dominate safety-critical areas.
Most recently, we are witnessing an ever-increasing reliance on \acp{CPS} that demands strict safety assurances.
To achieve safety assurances for a \ac{CPS}, one could formally specify the safety property of interest, and finally apply a model-based verification method to check the safety property should it be possible to model the \ac{CPS} formally.
Of note, formal modeling is a labor intensive and error-prone process whose difficulty level strictly depends on the complexity of the system.
Manual modeling is among the reasons formal verification methods becomes prone to human errors.
}

In \acp{CPS} embedded computers and networks control
physical processes. Most often, \acp{CPS} are interacting with their surroundings based on the context and the (history of) external events through an analog interface. We use the term hybrid system to refer to such reactive systems that intermix discrete and continuous components~\cite{MannaP92}.
Since hybrid systems are dominating safety-critical areas, safety assurances are of utmost importance. However, we know that most verification problems for hybrid systems are undecidable~\cite{Henzinger:HA}.
%

Therefore, models and model-based simulation play an essential role in the design process of such systems.
They help in identifying design problems as early as possible and facilitate integration testing with  model-in-the-loop techniques. 
%
However, the construction of hybrid models that comprise physical and digital behavior is challenging. Modeling such systems with reasonable fidelity requires  expertise in several areas, including control engineering, software engineering and sensor networks \cite{Derler&12}.  


\me
{
Most often, \acp{CPS} are interacting with their surroundings based on the context and the (history of) external events through an analog interface.
We use the term hybrid system to refer to such reactive systems that intermix discrete and continuous components~\cite{MannaP92}.
Since hybrid systems are dominating safety-critical areas, the demands for strict safety assurances hits an all-time high.
On the other hand, most verification problems for hybrid systems are undecidable~\cite{Henzinger:HA}. 
Verifying a hybrid system is even more difficult when it is black-box; \ie it provides no open access.
Although there are black-box learning methods to facilitate verification \cite{DBLP:journals/jalc/PeledVY02,Aichernig18:FMCAD}, they are inapplicable to black-box hybrid systems.
Therefore, model-based methods applicable in this domain like computation of reachable sets, abstraction refinement, and barrier certificates are inapplicable to black-box hybrid systems.
}

\me
{
It is customary to approach black-box hybrid systems using simulation-based verification methods; \eg random testing. 
Of note, these methods are incomplete because verification only holds for the applied test
cases. 
Simulation-based verification methods generate test cases through sampling the observation domain of the hybrid system semi-systematically.
Thus, properties of sampling methods directly affect the safety assurances. 
It is often the case that a rigorously tested hybrid system behaves unexpectedly in rare conditions because those were outliers of the observation domain. 
}

The learning of a behavior model from critical rare conditions will facilitate the verification tasks. Machine learning methods enable us to learn such behavior models agnostic about the details of the application domain. One requirement is that sufficient data of these rare conditions are available. To support a diverse data set of rare conditions \ac{MBT} can be exploited to guide data sampling.

%To learn a behavioral model for these rare conditions machine learning can be used. Unfortunately, high performing machine learning models require a sufficient amount of informative data. 
%To this end, \ac{MBT} is exploited to guide data sampling. 

\begin{figure}[!tb]
  \centering
  \resizebox{0.6\columnwidth}{!}
  {
    \input{Figures/workflow}
  }
  %\includegraphics[width=0.6\columnwidth]{Figures/workflow}
  \caption{Learning a behavior model of a black-box hybrid system.}\label{fig:flow}
\end{figure} 

\me
{
In this paper, we combine automata learning, \ac{MBT}, and machine learning to learn a behavior model from a black-box hybrid system. 
We can use the learned behavior model for multiple purposes including runtime enforcement or prediction(?).
\Cref{fig:flow} depicts the overall execution flow of our proposed setting.
Given a black-box hybrid system, we use automata learning to infer a discrete abstraction of the system.
Next, we investigate the inferred discrete automata for critical behaviors using model-based verification.
Once behaviors of interest are discovered, we use them to drive the hybrid system and determine its observable actions in a continuous domain. This process results in a behavioral dataset with high coverage of hybrid system's behavior including rare conditions. 
Finally, we use a machine learning method to train a \ac{RNN} model that generalizes behavioral dataset. 
For evaluation, we compared four different dataset generation approaches, by generating datasets, learning \ac{RNN} models from them and computing various performance measures for detecting critical behaviors in unforeseen situations. \textcolor{red}{Results show that testing strategies based on learned models outperform random dataset generation, \eg reducing the classification error by a factor of five given largest evaluated dataset size.} 
}

\subsection*{Motivating Example}
\me
{
Throughout the paper we illustrate our approach utilizing a platooning scenario.
%A hybrid platooning system consists of an embedded control system and a string of cars as the plant.
%\begin{itemize}
%\item What is the domain of observations; \ie \textbf{observable states}?
%\item What do we consider the track and the curves in the road \ie \textbf{is it part of the environment}?
%\item We need a schematic of the platooning system like the one presented %\href{http://www.cav2007.org/Docs/Fraenzle.HybridSystems.pdf}{\underline{here}}
%in slide 5.
%\end{itemize}
Platooning of vehicles is a complex distributed control scenario, see~\cref{fig:platooning}. Local control algorithms of each participant are responsible for reliable velocity and distance control. 
The vehicles continuously sense their environments, e.g. the distance to the vehicle ahead and may use discrete, i.e. event triggered, communication to communicate desired accelerations along the platoon~\cite{Dolk2017}. %In~\citeN{Dolk2017}, a hybrid system representation of the vehicle platooning scenario depicted in~\cref{fig:platooning} is derived based on control theoretic considerations.
Besides individual vehicle stability, the most crucial goal in controller design is to guarantee so-called string stability of the platoon~\cite{Ploeg2013}. 
This stability concept basically demands that errors in position or velocity do not propagate along the vehicle string which otherwise might cause accidents or traffic jams upstream.
Controllers for different platooning scenarios and spacing policies are available in literature, \eg constant time headway spacing ~\cite{Ploeg2013} or constant distance spacing with or without communication~\cite{Rupp2017}.
}
\begin{figure}[tb]
  \centering
  \includegraphics[width=\columnwidth]{Figures/platooningv2.pdf}
  \caption[Platooning as distributed control scenario.]{Platooning as distributed control scenario\footnotemark.}\label{fig:platooning}
\end{figure} 
\footnotetext{Adapted from a figure in~\cite{Dolk2017}.}


\me
{
Available controller designs are legitimated by rigorous mathematical stability proofs as an important theoretical foundation. In real applications it is often hard to fulfill every single modeling assumption of the underlying proofs, \eg perfect sensing or communication. However, these additional uncertainties can often be captured in fine-grained simulation models. This motivates \ac{MBT} of vehicle platooning control algorithms by the approach presented in this paper. Also, the learned behavior model can be used to detect undesired behavior during run-time. In~\cite{Dolk2017}, a hybrid system formulation of a platooning scenario is presented based on control theoretic considerations. In this contribution we aim to determine targeted behavior of such models with as few assumptions as possible by combining \ac{MBT} and machine learning. 
Since the relative distance between arbitrary chains of vehicles has been rigorously examined for our platooning scenarios (string stability has been verified), we concentrate on the absolute distance between two vehicles in the platoon, the leader and its first follower.
}

%\textcolor{red}
%{
%Would you please write a few lines to clarify how a plant is formed in a distributed control system.
%Are other controlled entities considered to be part of the adversarial environment?
%It would be great if we dive into the matter and also describe everything using a schematic figure.
%}


\me
{
\noindent\textbf{Outline.} This paper has the following structure.
\Cref{sec:preliminaries} summarizes automata learning and \ac{MBT}.
\Cref {sec:method} explains how to learn an automaton from a black-box hybrid system, then use it to target interesting behavior of the hybrid system such that we create a behavioral dataset that can be used for machine learning purposes.
\Cref{sec:results} discusses the results gained by applying our approach to a real-world platooning scenario.
\Cref{sec:related} covers related work.
\Cref{sec:conclusion} concludes and discusses future research directions.
}
